Power Redistribution for Optimizing Performance in MPI Clusters

Power efficiency has recently become a major concern in the high-performance computing domain. HPC centers are provisioned by a power bound which impacts execution time. Naturally, a tradeoff arises between power efficiency and computational efficiency. This paper tackles the problem of performance optimization for MPI applications, where a power bound is assumed. The paper exposes a subset of HPC applications that leverage cluster parallelism using MPI, where nodes encounter multiple synchronization points and exhibit inter-node dependency. We abstract this structure into a dependency graph, and leverage the asymmetry in execution time of parallel jobs on different nodes by redistributing power gained from idling a blocked node to nodes that are lagging in their jobs. We introduce a solution based on integer linear programming (ILP) for optimal power distribution algorithm that minimizes total execution time, while maintaining an upper power bound. We then present an online heuristic that dynamically redistributes power at run time. The heuristic shows significant reductions in total execution time of a set of parallel benchmarks with speedup up to 2.25x.

==> background.tex <==
%!TEX TS-program = make
%!TEX root = main.tex
\section{Background}
\label{sec:bg}



==> implementation.tex <==


